EVECTOR: An orchestrator for analysing attacks in electric vehicles charging system

Electric Vehicle (EV) charging infrastructure is critical for the widespread adoption of EVs, ensuring efficient and secure charging processes. Evaluating the security and performance of EV charging systems in real-world infrastructure poses significant challenges due to the diversity of information exchange between vehicles and charging stations/Electric Vehicle Supply Equipment (EVSE), including complex network protocols, scale of deployment and a variety of potential threats. Existing simulation frameworks are unable to handle complex security scenarios across these differing data exchange protocols. In this paper, we propose a novel EV orchestration framework: EVECTOR, which addresses the limitations of existing simulation systems by enabling both quantitative and qualitative analyses of EV charging scenarios. EVECTOR also provides a flexible attack orchestrator to simulate realistic attack behaviours on EV charging infrastructure. We validate the EVECTOR framework through two case studies: (a) cyber-physical attacks such as broken wire; and (b) cyber-specific attacks such as frame fuzzification. The case studies highlight the effectiveness of EVECTOR in providing deeper insights into the security and performance of EV charging systems.

==> TC/motivation.tex <==
\section{B\lowercase{ackground and motivation}}
\label{sec:motivation}

In this section, we first discuss the architectural details of GWA. We then analyse the challenges of deploying applications on geo-distributed environments. 

%\input{figuresTex/fig-motivation}



%Unlike the previous works~\cite{} that assume the network latency is already given or can be predicated based on the historical data; and based on the network latency, the response time is computable if the deployment solution is given. However, in our assumption that \emph{the network latency can only be obtained after the benchmark experiment, which is much more realistic.} Because the web developer may not have the access to all the datasets that record the historical data of the network latency across all available hosts. Even if the datasets are given, how to precisely predict and compute the response time for each user in a given deployment solution is grand challenge.




\input{figuresTex/fig-mot1} 

\subsection{Geo-distributed web-application}

%\myparagraph{GWA Architecture} 
A GWA follows a sophisticated architecture with a set of web servers deployed close to the users in order to provide low latency. Each web server may have a local database to cache the frequently visited contents. 
%It also ensures that sensitive data must not sent outside an specific location/region due to privacy and ethical issues \cite{voigt2017eu} imposed by that region. 
%Moreover, these user-interfaces are connected to one or more centralized databases with fast prefetching mechanisms. Finally, the GWA can be personalised on any device (e.g. desktop, mobile) according to the user requirements.}
%A GWA has a set of user-interfaces deployed close to users to achieve low latency, and each user-interface may have a local database to cache the frequently visited contents. 
Moreover, these web servers connect to one or more central databases, because moving a large volume of data is not easy and sensitive data must be stored at specific locations/regions due to privacy and ethical issues \cite{voigt2017eu}.



\myparagraph{Variety and uncertainty of deployment environment} Cloud computing provides an opportunity for WA owners to realize  global deployment. 
Since there are more than $267$ CPs available in the marketplace, offering numerous host configurations at each datacenter geo-location (e.g., AWS (Amazon Web Services) offers $275$ instances at the Europe (London) datacenter). Moreover, these hosts are inter-connected using WAN (Wide Area Network). However, the available bandwidth between a pair of DCs can be variable. The authors in \cite{viswanathan2016clarinet} reported that the ratio of the highest pair to the lowest pair bandwidth is greater than $20$ in both Amazon EC2 (Elastic Compute Cloud) and Microsoft Azure. 

\myparagraph{Location matters} The response time is dramatically affected by the location between user and the WA host. Fig. \ref{fig:mot1} shows a significant fluctuation of the response time when a WA is deployed in London and numerous users are accessing it from different geo-locations. \change{Here, $L_n$ represents the user's geolocation.} 
It shows that the highest latency is almost six times the lowest one.

\footnotetext{Data is available at: https://github.com/DNJha/Middleware2020}

% Additionally, Fig. \ref{fig:mot2} shows that with the fixed host capacity the latency increase dramatically when the host is saturated, i.e. when more than 2000 requests are sent simultaneously. 

%verifies that with same host and client, changing the number of requests changes the network delay and an increasing slope is visible (with some variance) with increasing number of requests.




\subsection{Deployment challenges}

\myparagraph{Importance of deployment location} Assume that a company wants to open its global business, starting to build a GWA. The central database is deployed at their headquarters inside the UK along with a web server. Due to limited budget, the company can only set up 
%ja_edit Should this be "one other"? done
one other web server which is deployed in China. Users from China can experience low latency by visiting this GWA. However, if many requests need to be redirected to the central database, users from China can experience huge latency because of the long-distance communication and limited bandwidth. However, there is no literature that has considered how to tackle this issue.



%Nowadays, the web-application is becoming complex and ones may have multiple tiers and each tier may be developed using wide range of technology stacks such as Java, JavaScrirpt .NET, PHP, MySQL, Neo4j.
%Consider a test web-application with users distributed globally as shown in Fig. \ref{fig:motivation}. To provide better user service, the available budget allows developer to  replicate $2$ copies of web server deployed at different geo-location connected to a centralized database server. Considering there are $5$ datacentre geo-locations (datacentre $A$ - $E$) available for the deployment of web-application components, one deployment solution is selected as shown in Fig. \ref{fig:motivation}. Here, the centralized database is installed at datacentre $B$ (New York, US) and the two web-servers are installed at datacentre $C$ (London, UK) and $E$ (Sydney, Australia). Now this solution is best suitable for user $3$ (UK) with the minimum response time as the network delay between user - web-server and web server - database server is minimal. For user $7$ (located in Perth), where the delay between user and web server is minimum while there is a significant delay between web server and database server and User 2 (Argentina) and User 4 (South Africa) with minimal delay between web-server and database server while substantial delay between user and web server, the response time is moderate. However, for user $5$ and $6$, the response time is worse as neither the web server is near to the user nor the database is near to the web-server. Therefore, the considered deployment solution is found to be non-optimial and unsuitable for the global users. 

\myparagraph{Importance of choosing host types} Users' experience (e.g., response time) is significantly dependent on the capacity of the hosts executing the GWA. Since the CPs offer numerous host configurations, the GWA owner may not have a clear idea of choosing suitable ones without executing them.
If the hosts can not provision sufficient computing resources, it will also cause high response time, or even outage problems. 
%ja_edit Sorry, I'm struggling with this next sentence - it seems to be saying that hiring more powerful resources can result in under-provisioning and "bring dramatically resource wastage" does not make sense (grammatically) but as I'm not sure what you were trying to say overall, I don't know what to suggest to fix it: done (updated the sentence)
In contrast, hiring powerful hosts may cause under utilization of computing resources, thus leading to resource wastage. As a results, the hosts must be evaluated before deploying the real GWA.    

\myparagraph{Benchmarking geo-distributed web-application} 
Benchmarking GWA is challenging from both \emph{system} and \emph{algorithm} perspectives. 
The \emph{system} challenge is that the ideal benchmark orchestrator is able to interact with various CPs that offer different ways to access their computing resources and automatically run the benchmark application on these resources, while providing the required evaluation results. However, most research is focused on single cloud scenarios \cite{cecchet2011benchlab, scheuner2015cloud}. \cite{jha2019smartdbo,jha2019cost} tackled the problem of deploying containerized web-applications on multiple clouds belonging to different CPs, but these tools fail to orchestrate a GWA benchmarking.

Regarding the \emph{algorithm} challenge, the desired orchestrator has to select the host from a mass of available candidates within a limited budget. This challenge is amplified when we aim to maximize the user's experience at global level. In other words, the orchestrator has not only to consider \emph{which} types of hosts should be benchmarked, but also \emph{where} to run the selected hosts. As a result, the proposed algorithm needs to have the following desirable properties. 

\noindent \textbf{Close to users.} The generated benchmarking solutions need to deploy the GWA close to its users, which is one of the important tricks for reducing the response time significantly.

\noindent \textbf{Increase the diversity of hosts.} \change{Depending upon the application type and the workload involved, a solution with a given host type and location may not be suitable. If we can evaluate more diverse deployment solutions, with varying underlying host configuration and location, we will have more opportunity to find a solution to satisfy QoS requirements}. 

\noindent \textbf{Consider the benchmarking time and budget.} 
To benchmark a GWA, the time and budget must be under consideration. Both directly influence how many \emph{selected} deployment solutions can be obtained.

%\zy{maybe put more if we have}


%\subsection{Benchmarking of geo-distributed web-application}
%To find an optimal deployment option for the web-application, benchmarking the host configuration is considered to be the best means. 
%To capture the behavior of web-applications, numerous benchmarks are proposed by academia \cite{scheuner2015cloud,chhetri2016smart,Cecchet:2011:BOT:2002168.2002172} and industry\footnote{https://cs.nyu.edu/~totok/professional/software/tpcw/tpcw.html}$^,${\footnote{https://www.wikibooks.org/} $^,$\footnote{https://cwiki.apache.org/confluence/display/OLIO/Index}}. There are three features of a benchmark to be emulated, (a) server-side feature, (b) workload generation and (c) workload injection \cite{curiel2018workload}.
%%The available benchmarks try to emulate the server-side features of the application along with workload generation and injection. 
%
%(a) \emph{server-side feature} is emulated in terms of domains, associated tiers and interactivity support. 
%Domain specifies the application type and the workload characteristics e.g. social media web application has different characteristics  as compared to finance or gaming web-application. Regardless of the complexity to capture the idiosyncrasies of every domain, it is necessary to consider as many domains as possible to make the  benchmark generic.  
%Multi-tier architecture support is provided in the form of MVC (Model View Controller) architecture which can be implemented using either traditional (e.g. JavaEE and ASP.NET) or modern (e.g. Python Django and Ruby on Rails) frameworks. Irrespective of the underlying framework, interactivity is supported by technologies such as jQuery and Angular that ease the user interaction allowing personalization on different devices.
% 
%(b) \emph{workload generation} is considered to capture the user interaction behavior with the web-application. Though a real trace-based benchmark \cite{Ratanaworabhan} can closely capture and mimic the  workload features, it is hard to generalize such benchmarks across multiple domains of web application. This is mainly due to the fact that a real trace can only represent a specific type of web application workload. Hence, there is need to find a balance between generalizability and specificity during the benchmarking process. This tension leads to the use of synthetic load generators that incorporates different user behaviors, e.g. think time and ramp up time to create sophisticated workloads \cite{4015510}. It also allows a fine-grained control over the setup features that characterize the workload.
%
%(c) \emph{workload injection} is traditionally perfomed using some replay tool such as httperf\footnote{https://github.com/httperf/httperf} that sends the simple or customized trace (combination of different traces) to the test application. This type of workload injection is very flexible as it allows to emulate hundreds (or more) users from a single host machine. However it may trigger DoS (Denial of Service) detection mechanism as all the request are generating from the same IP address and thus leads to the disruption of benchmark. A browser based workload injection is also available that uses Selenium supported browsers (Google Chrome, Safari, Firefox) to replay the workload. 
%
%
% 
%Though a real trace-based benchmark \cite{Ratanaworabhan} can closely capture and mimic the  workload features, it is hard to generalize such benchmarks across multiple domains of web applications. This is mainly due to the fact that a real trace can only represent a specific type of web application workload. Hence, there is need to find balance between generalizability and specificity during the benchmarking process.
%Using real data as a benchmark workload captures the best behavior however, it is specific only for particular application and is not easy to adapt or change according to the benchmark. 
%This tension leads to the use of synthetic load generators that incorporates different user behaviors, e.g. think time and ramp up time to create sophisticated workloads \cite{4015510}. To maintain a continuous stream of load, the trace is repeated using some replay tool e.g. httperf\footnote{https://github.com/httperf/httperf} that sends the simple or customized trace (combination of different traces) to the application. 
%
%Finally, the benchmark need to be orchestrated on the selected host configurations in the multi-cloud environment.
% Orchestrating the systematic deployment consists of following steps \cite{weerasiri2017taxonomy}: (i) defining the benchmark with their attributes and relationships, (ii) defining the host machine configuration (e.g., CPU cores, memory size, datacenter location, cost), (iii) instantiating the cloud host complying the application requirements, (iv) monitoring the resources to ensure the QoS and SLA parameters, and (v) controlling the overall processes. 
%Performing all these steps manually is tedious, error-prone and requires a lot of time and diverse knowledge of architecture and accessing mechanism of all these environments. 



%The web-application benchmark needs to be deployed on various host configurations in the multi-cloud environment.  Orchestrating the systematic deployment consists of following steps \cite{weerasiri2017taxonomy}: (i) defining the benchmark with their attributes and relationships, (ii) defining the host machine configuration (e.g., CPU cores, memory size, datacenter location, cost), (iii) instantiating the cloud host complying the application requirements, (iv) monitoring the resources to ensure the QoS and SLA parameters, and (v) controlling the overall processes. 
%Performing all these steps manually is tedious, error-prone and requires a lot of time and diverse knowledge of architecture and accessing mechanism of all these environments. 
%There are different frameworks available that automate/semi-automate the orchestration steps, however, they are limited only to single component web-application. 


%Built for Scale: You can manage a single instance or scale to thousands using AWS services. These services help you make the most of flexible compute resources by simplifying provisioning, configuration, and scaling

%\subsection{Background}\label{sec:background}
%
%To capture the behavior of web-applications, numerous benchmarks are proposed by academia \cite{scheuner2015cloud,chhetri2016smart,Cecchet:2011:BOT:2002168.2002172} and industry\footnote{https://cs.nyu.edu/~totok/professional/software/tpcw/tpcw.html}$^,${\footnote{https://www.wikibooks.org/} $^,$\footnote{https://cwiki.apache.org/confluence/display/OLIO/Index}}. These benchmarks try to emulate the server-side features of the application along with workload generation and injection. The server-side features are defined in terms of domain, different tiers and interactivity support \cite{Fielding:2017:RRA:3106237.3121282}. Multi-tier architecture support is provided in the form of MVC (Model View Controller) architecture which can be implemented using either traditional (e.g. JavaEE and ASP.NET) or modern (e.g. Python Django and Ruby on Rails) frameworks. Irrespective of the underlying framework, interactivity is supported by technologies such as jQuery, Angular and Underscore.js that ease the user interaction allowing personalization on different devices. 
%Workload generation and injection that captures the user interaction behavior is an important component of a benchmark \cite{curiel2018workload}. 
%Though a real trace-based benchmark \cite{Ratanaworabhan} can closely capture and mimic the  workload features, it is hard to generalize such benchmarks across multiple types of web applications. This is mainly due to the fact that a real trace can only represent a specific type of web application workload. Hence, there is need to find balance between generalizability and specificity during the benchmarking process.
%%Using real data as a benchmark workload captures the best behavior however, it is specific only for particular application and is not easy to adapt or change according to the benchmark. 
%This tension leads to the use of synthetic load generators that incorporates different user behaviors, e.g. think time and ramp up time to create sophisticated workloads \cite{4015510}. To maintain a continuous stream of load, the trace is repeated using some replay tool e.g. httperf\footnote{https://github.com/httperf/httperf} that sends the simple or customized trace (combination of different traces) to the application. 
%
%%Benchmarks such as Wikibooks\footnote{https://www.wikibooks.org/} (for wikipedia), Cloudstone's Olio\footnote{https://cwiki.apache.org/confluence/display/OLIO/Index} (for social media), TPC-W\footnote{https://cs.nyu.edu/~totok/professional/software/tpcw/tpcw.html} (for transactional web e-Commerce) are specific for particular domain whereas Benchlab \cite{cecchet2011benchlab} can support multiple domains altogether.
%
%The web-application benchmark needs to be deployed on various host configurations in the multi-cloud environment. Orchestrating the systematic deployment consists of following steps \cite{weerasiri2017taxonomy}: (i) defining the benchmark with their attributes and relationships, (ii) defining the host machine configuration (e.g., CPU cores, memory size, datacenter location, cost), (iii) instantiating the cloud host complying the application requirements, (iv) monitoring the resources to ensure the QoS and SLA parameters, and (v) controlling the overall processes. 
%
%\subsection{Related work}\label{sec:related}
%Performing all these steps manually is tedious, error-prone and requires a lot of time and diverse knowledge of architecture and accessing mechanism of all these environments. 
%There are different frameworks available that automate/semi-automate the orchestration steps. 
%%Some of the frameworks are cloud specific e.g. AWS CloudFormation\footnote{https://aws.amazon.com/cloudformation/} and Azure Resource Manager\footnote{https://azure.microsoft.com/en-gb/features/resource-manager/} while others are cloud agnostic e.g. Juju\footnote{https://jujucharms.com/}, Ansible\footnote{https://www.ansible.com/}. Frameworks such as Kubernetes (K8)\footnote{https://kubernetes.io/} and Docker Swarm\footnote{https://docs.docker.com/engine/swarm/} also handles the cluster management for containerized environment. 
%%There are also some frameworks specific for benchmarking e.g. CloudBench \cite{silva2013cloudbench}, Smart CloudBench \cite{chhetri2016smart}. However, none of the above discussed frameworks consider the optimized selection of benchmark and time execution time of the benchmark within the defined budget. The main limitations of the above discussed work are summarized below.  
%%Evaluating the system performance before the actual deployment has been studied extensively. TPC-W\footnote{https://cs.nyu.edu/~totok/professional/software/tpcw/tpcw.html}, WPBench \cite{zhang2009wpbench}, CloudStone \cite{sobel2008cloudstone}, Wikibooks\footnote{https://www.wikibooks.org/}, etc. are some common benchmarks for assessing the performance of web-application. Existing studies \cite{liew2012cloudguide,scheuner2018estimating,cecchet2011benchlab} uses these benchmarks to evaluate the performance of web-application in traditional VM environment. However, the containerized environment is different from the VM environment. 
%%With the growing demand of containers, studies also benchmark the performance of containers. 
%%Most of the existing studies 
%\cite{felter2015updated,Sharma:2016,kozhirbayev2017performance} evaluated the performance of containers for scientific applications where a few of them \cite{xavier2014performance,zhang2018comparative} evaluate for big data applications. 
%%However, in most of the works, the benchmarks configuration, host (VM/container) configuration and set up, benchmark execution and result collection is performed manually. 
%However most of these works are intended for single cloud environment, without considering the complexity of interacting with various APIs/SDKs provided by different cloud providers. 
%%It is not handy to perform all these operations by our own in multi-cloud environment as each cloud provider have specific APIs/SDKs for interaction. 
%
%There are few existing frameworks that handle the orchestration of benchmarks in multi-cloud environment. CloudBench \cite{silva2013cloudbench} and Smart CloudBench \cite{chhetri2016smart} automates the benchmark execution in multi-cloud environment. However, it is not easy to define the benchmarks using these frameworks. Also they are not specific for containerized environment. Additionally, Varghese et al. proposed a framework called DocLite \cite{varghese2016doclite} to evaluate the performance of VMs using containerized microbenchmarks. Microbenchmarks are executed on different VMs and the ranking is evaluated by using the set of weights provided by the user for different system parameters. This framework is specific for scientific application and may not be applicable for web application. Our proposed SmartDBO orchestrates the benchmark for web-application while allowing users to define and deploy the benchmark in a very interactive and user-friendly way.
%
%Additionally, there are some commercial tools,  e.g. CloudHarmony\footnote{https://cloudharmony.com/}, cloudorado\footnote{https://www.cloudorado.com/cloud\_server\_comparison.jsp}, Cloud Spectator \footnote{https://cloudspectator.com/}. available that perform the benchmark for users but they are not specific for particular applications. Also, they do not provide all the required metrics specific to that particular application for making proper decisions before final resource selection and provisioning. The limitations of the existing work are briefly summarized as follows.
%
%%Performing benchmark is very expensive but none of the available work considers the cost of benchmark. Also, benchmarking host for long time gives more accurate evaluation but imposes high cost and is not always suggested. In this work, we are not only allowing the automatic orchestration of the benchmark but also furnish user to find a set of benchmark that can cover as much diversity as possible within the defined budget. Our benchmark orchestration is based on Infrastructure as a code that allows user to reuse the available code to ease their deployment. 
%
%
%%\zy{review the important works related to web application benchmark and benchmark orchestrator}

%
%\myparagraph{Limitations} The cloud providers provide the shared and virtualized computing resources to their customers, which makes the cloud environments dynamic and the SLA very hard to guarantee \cite{serrano2016sla}. Moreover, the web application is very sensitive to the dynamically changing environment that directly affect user's satisfaction. Capturing or monitoring the changing behavior of the cloud environments requires the users to run their benchmark applications over a considerable time, which is very costly.    
%The existing benchmark applications/tools are not able to solve the trade-off between the limited budgets and the long-time benchmarking experiments.  
%
%Additionally, the variety of cloud providers offer a massive configuration choices of host. For instance, Amazon EC2 provides $43$ types of host for their customers\footnote{https://aws.amazon.com/ec2/instance-types/} excluding self customized hosts. It is not possible to run the benchmark applications over all available resources. The state-of-the-art systems do not consider this case that provides an optimized recommendation to help users in selecting the hosts from the massive number of available hosts spanned across multiple cloud providers.
%
%\subsection{Design goals}\label{sec:design-goal}
%
%To overcome the limitations discussed in the previous subsection, our proposed \projecttitle framework follows the three main design goals:
%
%\begin{itemize}
%	\item We want to automatically orchestrate \emph{any} containerized benchmark application across multi-cloud environments based on the users' specification. This will remove the huge burden from user side, i.e. the users do not need to  manually deploy the benchmark applications and define the benchmark  plans  over various cloud datacenters.  
%	\item We want to capture the dynamicity and the uncertainty of the cloud environment while ensuring the cost does not exceed the users' budget. This dynamicity and uncertainty may affect the performance of web-application, therefore reducing users'  satisfaction \cite{hoxmeier2000system}. 
%%	For example,  This is important for web applications because the response time of a website is significantly affecting user satisfaction \cite{hoxmeier2000system}.  
%	
%	\item We should be able to find an optimal set of hosts for benchmarking in a fixed budget that covers the diversity, in terms of host configurations, both within a cloud provider and across the cloud providers. This feature improves the chance for a user to find the best mix of hosts for deploying their web-applications. In other words, with our design the users has more chance to find the cheaper hosts which meet the performance requirements of their web applications. 
%\end{itemize}
%
%%\input{figuresTex/fig-shortterm}
%
%%\input{figuresTex/fig-longterm}






==> TC/optimization.tex <==
\section{Optimising the deployment}
\label{sec:opt}


This section presents a detailed description of the proposed approach which consists of the following four main components: \emph{(A) clustering}, \emph{(B) budget allocation}, \emph{(C) deployment solution generation}, and \emph{(D) benchmarking in real-world environments}. 


\subsection{Overview of executing \projecttitle}
To obtain the ``best'' deployment solution, each component is executed sequentially as shown in Alg. \ref{Algo2} and Fig. \ref{fig:mainalg}. An input set should be provided, in which the GWA and benchmarking budget $\mathcal{B}$ are provided by the user. The host information $\mathbb{V}_\RES$, including the CPU, memory, location and price, about each provider is pre-collected. In the first step, we partition the hosts into $K$ clusters (see Alg. \ref{Algo2} Line \ref{lineA1}). Next, the given budget $\mathcal{B}$ is allocated to $K$ clusters in step $2$ (Alg. \ref{Algo2} Line \ref{lineA2}). In step $3$, based on the allocated budget, clustered hosts and other provided information, a set of deployment solutions is generated (see Alg. \ref{Algo2} Line \ref{lineA3}). The obtained solutions are automatically deployed and executed on the corresponding hosts (step $4$). Finally, the benchmarking results are collecte,d and then a report is generated and sent back to the user (illustrated in Alg. \ref{Algo2} Line \ref{lineA4}). The following subsections indicate the technical details of each key component. 


\input{algorithm/alg_main.tex}

\input{figuresTex/fig-mainalg}

 
\begin{algorithm}[t!]
 \KwIn{
 $K_\textit{max}$ - maximum cluster size,
 $\mathbb{V}_\RES$ - cloud hosts
 }

\KwOut{
$\mathbb{C}\textit{lus} = \{\textit{Clus}_1,\dots, \textit{Clus}_K\}$ - obtained clusters
}

{\commentfontsize // {Apply Elbow method to get the optimal $K$}}
 
 \For{$  k=2,\dots, K_\textit{max}$}{
 
 {\commentfontsize // {Apply \textsc{K-means} }}
 
 $\textit{Clus}_k \gets \textsc{K-means}(\mathbb{V}_\RES, k)$

 {\commentfontsize // {Compute Intra-Cluster Variation   }}
 
 $\textit{ICV}_k \gets \sum_{j = 1}^k \sum_{a_i \in \textit{Clus}_j} ||a_i - u_j||^2$ \label{line_icv}
 }
 
 {\commentfontsize //{Find the knee point}}
 $\Delta \textit{ICV}_{k,k+1} \gets |\textit{ICV}_{k+1} - \textit{ICV}_k|$ ~
 for each $k < K_\textit{max}$
 
 $K = k(\textit{kneed}_{k, k+1} (\Delta \textit{ICV}_{k,k+1}))$ \label{icvk_diff}

 {\commentfontsize // {Find the final cluster}}
 
 $\mathbb{C}\textit{lus} \gets$ \textsc{K-means}$(\mathbb{V}_\RES, K)$



 \vspace{1em}
 \setcounter{AlgoLine}{0}
\kwfn{\textsc{K-means} ($\mathbb{V}_\RES, K$)}
 
 {\commentfontsize // {Initialise cluster center}}

 $u_k \gets$ {\tt rand} $(v_i) $~~for $ v_i \in \mathbb{V}_\WEB$ and  $ k \in K$ \label{center}
 
 
 \While{!~\textit{terminate}}{
 
 {\commentfontsize // {$v_i$ is allocated to a cluster}}
 
 \For{ each $ v_i \in \mathbb{V}_\WEB$}{
 
 $c_{ik} \gets
 \left\{
 \begin{array}{l}
  1  \hspace{0.5em} if \hspace{0.5em}  l = arg \hspace{0.5em} \underset{j}{min} ||v_i - u_k||^2 	 \\
  0  \hspace{0.5em} otherwise
 \end{array}
 \right. 
 $  \label{argmin}
 
 }
 
 
 {\commentfontsize //{Update the cluster center}}
 
 \For{$ k=1,\dots, K$}{
 
 $u_k \gets \frac{\sum_i (c_{ik} \times v_i)}{\sum_i c_{ik}}$ \label{update_center}
 }  
 }
 
\caption{\bf  Clustering algorithm}
\label{K-means-algo} 
\end{algorithm}

 

\subsection{Clustering}\label{sec:clustering}

Our first step is to create a set of clusters to partition the nodes in $\mathbb{V}_\RES$, i.e., each node $v_\RES^i \in \mathbb{V}_\RES$ is mapped to exactly one cluster with all the nodes belonging to the same cluster bearing similar host type characteristics ($h \in \mathbb{H}$). Each host type $h$ is associated with many aspects of resources such as CPU, memory, storage, bandwidth, etc. In this paper, the clustering algorithm considers CPU and memory properties. 
We employed \textsc{K-means} algorithm to create $K$ disjoint clusters $\mathbb{C}\textit{lus} = 
\{\textit{Clus}_1,\dots, \textit{Clus}_K\}$ \cite{kanungo2002efficient}. 

Note that the parameter $K$ needs to be found and input to the \textsc{K-means} algorithm, and determining $K$ is essential to achieve optimal partitioning. We employed the \emph{Elbow Method} to find this value~\cite{masud2018nice}. It receives $K_\textit{max}$ as input and 
starts with different values of $k \in \{0, 1, ..., K_\textit{max}\}$ and computes a total \emph{Intra Cluster Variation} $\textit{ICV}_k$ for each cluster size $k$ (Alg. \ref{K-means-algo} Line \ref{line_icv}). 
 The difference between $\textit{ICV}_k$ and $\textit{ICV}_{k+1} $ is determined for all $k, k+1$ and the knee point is detected using $\textit{kneed}$ library (Alg. \ref{K-means-algo} Line \ref{icvk_diff}). The resulting value of $K$ represents the optimal cluster number.
 
K-means clustering is then performed on the obtained cluster size $K$. Initially, each cluster $\textit{Clus}_k$ is assigned to an arbitrary cluster center $u_k$ (Alg. \ref{K-means-algo} Line \ref{center}). A data point $v_i$ including CPU and memory information is allocated to a cluster $\textit{Clus}_k$ based on the closeness to the cluster centre $u_k$ as shown in Alg. \ref{K-means-algo} Line  \ref{argmin}. 
Here, $||\cdot||$ represents the function (Euclidean function) to measure the distance between the data point $v_i$ and the cluster center $u_k$. The value $c_{ik}$ can be either $1$ if $v_i$ is allocated to cluster $\textit{Clus}_k$ or $0$ otherwise. With each iteration, $u_k$ is also updated (Alg. \ref{K-means-algo} Line \ref{update_center}). 
These steps are repeated until the termination condition is reac,hed which in our scenario that  is the cluster center $u_j$ remains unchanged.


The pseudo-code for the clustering algorithm is given in Algo.\ref{K-means-algo}.
It is worth mentioning that the clustering stage is performed only once on a host data set. The stage is repeated only when the dataset is changed. 


 
\subsection{Budget allocation}

As we discussed above, deployment solutions are generated for each cluster, so it is necessary to fairly distribute the given budget $\mathcal{B}$ to the clusters $\mathbb{C}\textit{lus}$.

Since the unit execution cost $\mathcal{P}(v_\RES^i)$ of host $v_\RES^i$ varies from one cluster to another, it is not suitable to divide the budget $\mathcal{B}$ equally among the clusters. The average cost for benchmarking a cluster is a good reference for budget distribution to ensure fairness. 
However, evaluating the average cost for a cluster requires computing the cost of each possibl,e solution which is not feasible otherwise.  
Alternatively, we use the mean of solutions which have the maximum and minimum cost as the reference to distribute the budget $\mathcal{B}$. To this end, we interact our Alg. \ref{Algo3} with the \emph{\textit{APSO}} (discussed in Section \ref{pso}).
For each cluster $\textit{Clus}_k \in \mathbb{C}\textit{lus}$, we first obtain a solution with maximum cost $\mathcal{C}_\textit{max}^k$ and minimum cost $\mathcal{C}_{min}^k$ by setting the optimisation constraint $\zeta$ as \textit{maximisation} and \textit{minimisation} respectively (see Alg. \ref{Algo2} Line \ref{lineB1}-\ref{lineB4}). 
Next, the average cost for each cluster $k$, $\mathcal{C}_{av}^k$ is computed by normalising the maximum and minimum cost (Alg. \ref{Algo2} Line \ref{lineB5}).
Finally, the user's budget $\mathcal{B}$ is distributed to each cluster $\textit{Clus}_k$ using the equation 
in (Alg. \ref{Algo2}  Line \ref{lineB6}) and $\mathcal{B}_k$ is returned.


\input{algorithm/alg_budget.tex}


\subsection{Deployment solution generation}

\input{algorithm/alg_solution}

In this stage, the cluster budget $\mathcal{B}_k$ is distributed to find a set of solutions for each cluster $\textit{Clus}_k$ as given in Alg. \ref{Algo4}. First, we generate $\eta$ set of solution $\mathbb{P}_k$ for each cluster $k$ using the \textit{APSO} algorithm (Line \ref{l3}). Next, each solution $\mathbb{P}_k[i_k]$ is added individually to a final list $\Theta_k^{fin}$ till no solution can be added in the remaining budget $\mathcal{B}_k^{left}$ (Line \ref{l6}). 
To maximise the utilisation of the budget, we combine all the remaining cluster budget $\mathcal{B}_k^{left}$ (Line \ref{l10}). Later, the budget $\mathcal{B}^{left}$ is allocated to each cluster in descending order based on its reference (refer to Alg. \ref{Algo2} Line \ref{lineB5}) to compute more solutions (Line \ref{l12}-\ref{l16}). Finally, the clustered solutions $\Theta_k^{fin}$ from each $k$ cluster are merged to get the final list of solution $\Theta'$ for the real deployment.



\subsection{Benchmarking in real-world environments} \label{real_}
The solutions $\Theta'$ obtained in the previous step are deployed using the \emph{deployment orchestrator} discussed in Section \ref{sec:architecture}. 
\change{To execute an optimised solution $\theta$, first the \emph{resource provisioner} extracts the host information including 
% specified cloud provider $c \in \mathbb{C}$ and 
instance configurations ($h$, $loc$ and $p$). Next, communication is established with the instance. The communication is performed using cloud-specific APIs defined in the \emph{Go} language. After the successful initialisation of GWA hosts, each host is installed with the specific Docker images and communication is established between various GWA components.

A similar process is followed to initiate the client hosts required for the \emph{load generator}. The \emph{deployment orchestrator} is notified with the successful establishment of GWA and client hosts. Following this, the state of deployment, along with the IP address of the hosts is returned. 

With the successful establishment of GWA hosts, the client hosts are launched with the defined \emph{test plan} and the IP address of the web server GWA components. Since there are multiple web server GWA components, a simple \emph{geo-location rule-based load generation} was developed, i.e., the client will load the nearest web server host in terms of geo-location. The client hosts are triggered to load the web server hosts and the execution starts. 

The completion of an experiment is reported to the \emph{deployment orchestrator} and the \emph{result aggregator} retrieves the results from the clients. The hosts are terminated and the cloud resources are released. Finally, the \emph{result aggregator} compares all the results and returns the best solution $\theta^{best}$ to the user.} 


\subsection{Complexity analysis} \label{sec:complexity1}
This section computes the worst-case time complexity of our proposed framework, \projecttitle. \projecttitle consists of four main components as given in Fig.\ref{fig:mainalg}, the complexity of \emph{clustering}, \emph{benchmarking in real-world environment} is \emph{O(1)}. The complexity of \emph{budget allocation} and \emph{deployment solution generation} depends on the complexity of \textit{APSO}. In our case, the complexity of \textit{APSO} depends on the population space $s << |\mathbb{V}_\RES|$, number of GWA components $|\mathbb{V}_\WEB|$ and the maximum number of iteration before termination $\kappa$ is given as $ O((s + s \log s + \kappa) \times |\mathbb{V}_\WEB|)$. 
Here, $\kappa$ and $s$ are constant thus reducing the complexity of \textit{APSO} to be $O(|\mathbb{V}_\WEB|)$.
 
Since the number of clusters $K$ is a constant, the complexity of \emph{budget allocation} and \emph{deployment solution generation} are also equal to $O(|\mathbb{V}_\WEB|)$. Therefore, the overall worst-case complexity of our proposed approach is $O(|\mathbb{V}_\WEB|)$. The result is also validated with real experiments as given in Section \ref{sec:scalable}. 


 

==> TC/overview.tex <==
\section{System overview}
\label{sec:overview}   
This section describes the GWA deployment model and formalises the candidate selection problem to an optimisation problem.

\begin{table}[t]
 \centering 
 \caption{A summary of symbols used in the paper}
 \label{tab:symbol}
 \resizebox{\columnwidth}{!}{
 % \begin{adjustbox}{max width=\columnwidth}
 \begin{tabular}{|l|l|}
 \hline
 \textbf{Symbols} & \textbf{Description} \\ \hline
 $\mathbb{G}_\WEB = (\mathbb{V}_\WEB, \mathbb{E}_\WEB)$ & Graph of GWA \\ \hline 
 $\mathbb{G}_\RES = (\mathbb{V}_\RES, \mathbb{E}_\RES)$ & Fully connected graph of cloud provider hosts \\ \hline
 $v_\RES^i \in \mathbb{V}_\RES$ & Host $i$ of $\mathbb{G}_\RES$ \\ \hline 
 $h_{v_\RES^i} \in \mathbb{H}$ & Host type for host $v_\RES^i$ \\ \hline
 $loc_{v_\RES^i} \in \mathbb{L}$ & Datacenter geo-location for host $v_\RES^i$ \\ \hline
 $\theta \in \Theta$ & A deployment mapping/solution in the set of solutions $\Theta$ \\ \hline
 $\mathcal{P}(\theta^\mathbf{h}(v_\WEB^i))$ & Unit execution cost for host mapping $\theta^\mathbf{h}(v_\WEB^i)$ \\ \hline
 $\mathcal{O}(v_\WEB^i)$ & Total execution time of $v_\WEB^i$ \\ \hline
 $\mathcal{N}(\theta^\mathbf{h}(v_\WEB^i), \theta^\mathbf{h}(v_\WEB^j))$ & Unit data transfer cost from $\theta^\mathbf{h}(v_\WEB^i)$ to $\theta^\mathbf{h}(v_\WEB^j)$ \\ \hline
 $\mathcal{D}(v_\WEB^i, v_\WEB^j)$ & Size of data transferred from $v_\WEB^i$ to $v_\WEB^j$ \\ \hline
 $\mathcal{C}_\textit{exe}^{\theta}, \mathcal{C}_\textit{com}^{\theta}$ & Execution cost and transfer cost for a solution $\theta$ \\ \hline
 $\mathcal{C}^{\theta}$ & Total cost of a solution $\theta$ \\ \hline
 $\Theta'$ & Optimal subset of $\Theta$ \\ \hline
 $\mathcal{B}$ & User's budget \\ \hline
 $s$  & Population of particle \\ \hline
 $\mathbb{P}, \mathbb{P}^{local}, \mathbb{V}el$ & Set of position, local best position and velocity of particles \\ \hline
 $\mathbb{P}_{best}^{global}$ & Global best position vector \\ \hline
 $\zeta$ & Optimisation objective (maximise or minimise) \\ \hline
 $\mathbb{P}_{final}$ & Output solution set \\ \hline
 $\eta = |\mathbb{P}|_{final}$ & Number of output solution \\ \hline
 $\omega$ & Inertia weight \\ \hline
 $C1, C2$ & Self recognition and social constant factor \\ \hline
 $K, K_{max}$ & Optimal and maximum cluster size \\ \hline
 $\mathbb{C}lus = \{Clus_1, \dots, Clus_K\}$ & $K$ disjoint clusters \\ \hline
 $u_j$ & Data point representing cluster center for $Clus_j$ \\ \hline
 $a_i$ & Data point representing host $v_\RES^i$ \\ \hline
 \end{tabular}
 % \end{adjustbox}
}
\end{table}
 

\subsection{Web-application deployment model}
\label{sec:model}
A GWA is given as a directed graph 
$\mathbb{G}_\WEB = (\mathbb{V}_\WEB, \mathbb{E}_\WEB)$, where the nodes $\mathbb{V}_\WEB=\{v_\WEB^1,\dots,v_\WEB^n\}$ represent the web application components (microservices), and the arcs $\mathbb{E}_\WEB$ represent the dependency between components, including data flow and transactions. 

The computing resources  are given as a complete directed graph 
$\mathbb{G}_\RES = (\mathbb{V}_\RES, \mathbb{E}_\RES)$, 
where the nodes $\mathbb{V}_\RES=\{v_\RES^1,\dots,v_\RES^m\}$ 
represent available hosts and 
the edges $\mathbb{E}_\RES$ represent the network connections among the hosts.
For each host $v_\RES^i\in\mathbb{V}_\RES$:
\begin{itemize}
\item 
$h_{v_\RES^i} \in \mathbb{H}$ is the host type of $v_\RES^i$,
\item 
$\textit{loc}_{v_\RES^i} \subseteq \mathbb{L}$ is a nonempty set of datacenter geo-locations
of $v_\RES^i$,
\item 
$\mathcal{P}(v_\RES^i)$ is the unit execution cost of $v_\RES^i$,  
\item
$\mathcal{N}(v_\RES^i,v_\RES^j)$
is the unit data transfer cost from  $v_\RES^i$ to another host $v_\RES^j\in\mathbb{V}_\RES$.
\\
Note that we may have 
$\mathcal{N}(v_\RES^i,v_\RES^j)\neq\mathcal{N}(v_\RES^j,v_\RES^i)$. 
\end{itemize} 

To model deployments of web applications to cloud providers, we use \emph{deployment}  
mappings $\theta:\mathbb{V}_\WEB \to \mathbb{V}_\RES\times \mathbb{L}$
and denote 
$\theta(v_\WEB^i)=(\theta^\mathbf{h}(v_\WEB^i), 
\theta^\mathbf{l}(v_\WEB^i))$, for every GWA component $v_\WEB^i$.
We also require that the following are satisfied, for all distinct
GWA components  $v_\WEB^i$ and $v_\WEB^j$:
\begin{itemize}
\item 
$\theta^\mathbf{l}(v_\WEB^i)\in \textit{loc}_{\theta^\mathbf{h}(v_\WEB^i)}$, 
\item 
$h_{\theta^\mathbf{h}(v_\WEB^i)}=h_{\theta^\mathbf{h}(v_\WEB^j)}$, 
\item  
$\theta^\mathbf{h}(v_\WEB^i)\neq \theta^\mathbf{h}(v_\WEB^j)$ 
and 
$\theta^\mathbf{l}(v_\WEB^i)\neq \theta^\mathbf{l}(v_\WEB^j)$ .
\end{itemize}  
The set of all   
deployment mappings is denoted by $\Theta$. 
Figure~\ref{fig:model} shows an example of one of the solutions $\theta$.
\\
Note that, for a deployment mapping, the host types of hosts
allocated to all the GWA components do not differ. 
Moreover, the  hosts and locations allocated to distinct components 
must be different. 


Table~\ref{tab:test2} shows the possible number of deployment 
mappings by varying the numbers of GWA components and hosts,
assuming that there is only one host type, and that each host has only one geo-location
(in such a case, there are exactly
$n!\cdot\binom{m}{n} = n!\cdot\frac{m!}{n!(m-n)!}=\frac{m!}{(m-n)!}$ different deployment mappings). 
Note that even for relatively small numbers of GWA components $n=30$ and
hosts $m=50$, the number of possible deployment mappings is overwhelming, and so the selection of optimal deployment mappings cannot be done by any brute-force approach. 
 

\begin{table}[b]
\centering 
 \caption{Number of deployment mappings generated by varying the number of GWA components and the number of hosts}
 \label{tab:test2}
 % \resizebox{\columnwidth}{!}{
\begin{tabular}{|c|ccccc|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}GWA \\ comp.\end{tabular}}} & \multicolumn{5}{c|}{\textbf{Number of hosts}} \\ \cline{2-6} 
& \multicolumn{1}{c|}{\textbf{30}} & \multicolumn{1}{c|}{\textbf{35}} & \multicolumn{1}{c|}{\textbf{40}} & \multicolumn{1}{c|}{\textbf{45}} & \textbf{50} \\ \hline
\textbf{5} & \multicolumn{1}{c|}{2.E+07} & \multicolumn{1}{c|}{4.E+07} & \multicolumn{1}{c|}{8.E+07} & \multicolumn{1}{c|}{1.E+08} & 3.E+08
\\ \hline
\textbf{10} & \multicolumn{1}{c|}{1.E+14} & \multicolumn{1}{c|}{7.E+14} & \multicolumn{1}{c|}{3.E+15} & \multicolumn{1}{c|}{1.E+16} & 4.E+16
\\ \hline
\textbf{15} & \multicolumn{1}{c|}{2.E+20} & \multicolumn{1}{c|}{4.E+21} & \multicolumn{1}{c|}{5.E+22} & \multicolumn{1}{c|}{5.E+23} & 3.E+24
\\ \hline
\textbf{20} & \multicolumn{1}{c|}{7.E+25} & \multicolumn{1}{c|}{8.E+27} & \multicolumn{1}{c|}{3.E+29} & \multicolumn{1}{c|}{8.E+30} & 1.E+32
\\ \hline
\textbf{25} & \multicolumn{1}{c|}{2.E+30} & \multicolumn{1}{c|}{3.E+33} & \multicolumn{1}{c|}{6.E+35} & \multicolumn{1}{c|}{5.E+37} & 2.E+39
\\ \hline
\textbf{30} & \multicolumn{1}{c|}{3.E+32} & \multicolumn{1}{c|}{9.E+37} & \multicolumn{1}{c|}{2.E+41} & \multicolumn{1}{c|}{9.E+43} & 1.E+46\\ \hline
\end{tabular}
% }
\end{table}
 
\input{figuresTex/fig-model}
 
\subsection{Problem formulation}
\label{sec:problem} 

Our approach is first to identify a possibly widest range of deployment options with varying host types and locations adhering to the available budget, and then to benchmark these to obtain an optimal deployment. We formulate such a \emph{two-phase} approach in the following way.
 
\myparagraph{Phase I} 
We aim to find the largest set of deployment mappings with the total cost within a given budget $\mathcal{B}$. 


For each deployment mapping $\theta\in\Theta$, we consider two types of costs (in terms of time), namely the \emph{execution} cost $\mathcal{C}_\textit{exe}^\theta$, and the \emph{communication} cost  $\mathcal{C}_\textit{com}^\theta$, as shown in Eq.\ref{eq:1}, where $\mathcal{O}(v_\WEB^i)$ is the total execution time for a GWA component $v_\WEB^i$ and $\mathcal{D}(v_\WEB^i,v_\WEB^j)$ is the size of data transferred from a GWA component $v_\WEB^i$ to another GWA component $v_\WEB^j$. The cost model is based on the Pay-As-You-Go pricing model. The choice of the Pay-As-You-Go model is based on the wide adoption by all cloud providers, which makes the cost model generalised.

\begin{equation}
\label{eq:1}
\begin{array}{lcl}
\mathcal{C}_\textit{exe}^\theta 
&=& 
\displaystyle\sum_{i=1}^n \mathcal{O}(v_\WEB^i) \cdot 
\mathcal{P}(\theta^\mathbf{h}(v_\WEB^i)) \\
\mathcal{C}_\textit{com}^\theta 
&=&
\displaystyle\!\!\!\!\!\!  \sum_{i, j=1\wedge i\neq j }^n \!\!\!\!\!\!\! 
\mathcal{D}(v_\WEB^i,v_\WEB^j) 
\cdot 
\mathcal{N}(\theta^\mathbf{h}(v_\WEB^i), \theta^\mathbf{h}(v_\WEB^j)) \\
\mathcal{C} ^\theta 
&=&
\mathcal{C}_\textit{exe}^\theta + \mathcal{C}_\textit{com}^\theta
\end{array}
\end{equation}
We then formulate our goal as an optimisation problem given by Eq.~\ref{eq:obj1} 
together with the formulas for deployment costs given by Eq.~\ref{eq:1}. 
 
\begin{equation} 
\label{eq:obj1}
\begin{array}{l}
{\textbf{maximize:}}~~~ 
|\Theta'| ~~~\textit{where}~ \Theta'\subseteq\Theta \\[2mm]
\textbf{subject to:}~~~ 
\displaystyle\sum_{\theta\in\Theta'} \mathcal{C}^\theta  \leq \mathcal{B} 
\end{array}
\end{equation}

 
\myparagraph{Phase II} In this phase, the set of deployment mappings $\Theta'$ obtained in Phase~I is deployed and executed on a real-cloud environment with the execution results being collected. The deployment mapping with
the ``minimal" response time is then selected and used for the actual deployment of GWA components.


==> TC/pso.tex <==
\section{Adaptive PSO algorithm}
\label{pso}

Particle Swarm optimisation (\textit{PSO}) is a well-known optimisation algorithm used to find a solution in a multidimensional space \cite{kennedy1995particle}. However, in the high-dimensional space, the convergence rate is low with the chance of falling into local optima. Numerous updated versions of \textit{PSO} have been proposed for task scheduling in the cloud environment, e.g., Nested PSO \cite{song2020scheduling}, Multitask PSO \cite{han2023multitask}.


In this section, we propose \emph{Adaptive Particle Swarm Optimisation (\textit{APSO})} algorithm which is able to find a solution without getting stuck in the local optima. The primary novelty of \textit{APSO} lies in its adaptive mechanism, which dynamically adjusts its parameters during optimisation based on problem characteristics and search progress. This contrasts with traditional algorithms like Genetic Algorithms (\textit{GA}) and Ant Colony Optimisation (\textit{ACO}) that employ fixed parameters, potentially hindering their performance in complex multi-cloud scenarios. Compared to these traditional algorithms, \textit{APSO} offers several advantages in terms of scalability, solution quality, and convergence speed as given below:
\begin{itemize}
 \item 
 Scalability: \textit{APSO}'s adaptive nature empowers it to efficiently handle large-scale optimisation problems with numerous decision variables and constraints, a common challenge in multi-cloud environments. Traditional algorithms like \textit{GA} and \textit{ACO} may struggle with scalability, leading to increased computational costs or suboptimal performance. 

 \item
 Quality: By balancing exploration and exploitation through its adaptive mechanism, \textit{APSO} frequently discovers higher-quality solutions, often reaching global or near-optimal configurations. This surpasses algorithms like \textit{GA} and \textit{ACO}, which can suffer from premature convergence or slower convergence rates, resulting in less optimal solutions.

 \item
 Convergence: \textit{APSO}'s adaptive parameter tuning and efficient search space navigation often lead to faster convergence compared to \textit{GA} and \textit{ACO}. This advantage translates to quicker solutions, particularly valuable in time-sensitive optimisation tasks within multi-cloud environments. 
\end{itemize}

Alg.\ref{Algo1} illustrates the key steps of the proposed \textit{APSO}.
In concrete terms, we first initialise three sets of vectors, each having $s$ elements: 
\[
\begin{array}{lcl}
\mathbb{P} &=& \{\vec{P_1}, \dots, \vec{P}_{s}\}
\\
\mathbb{P}^\textit{local} &=& \{\vec{P}^\textit{local}_1, \dots, \vec{P}_{s}^\textit{local}\}
\\
\mathbb{V}\textit{el} &=& \{\vec{\textit{Vel}}_1, \dots, \vec{\textit{Vel}}_{s}\}
\end{array}
\] 
$\mathbb{P}$ records the set of current deployment solutions; each $\vec{P}_i$ represents a deployment mapping $\theta_i$. $\mathbb{P}^\textit{local}$ stores the best deployment solution obtained for each $\vec{P}_i$ during any run-time iteration. 
In $\mathbb{V}\textit{el}$, each $\vec{\textit{Vel}}_i$ represents the vector variable to update the value of $\vec{P}_i$. 

We initialise $\vec{P}_i$ by randomly mapping a host from $\mathbb{V}_\textit{res}$ for each component of the GWA. 
% (for the sake of simplicity, we assume that each host has just one location). 
The generated $\vec{P}_i$ is checked for the validity of the deployment mapping using a \emph{Valid Particle Generator (VPG)} as specified by the constraints in Section~\ref{sec:problem} and retained only if it is found valid (Alg.\ref{Algo1} Line~\ref{lineP2}-\ref{lineP4}). 
Otherwise, it is discarded and, eventually, a valid deployment mapping is derived. 
Then, $\mathbb{P}^\textit{local}$ is assigned  $\mathbb{P}$ for all $s$ components.
\\
To allow a uniform update of the current deployment solution $\vec{P}_i$ to a new $\vec{P}_{i}^\textit{new}$, $\vec{\textit{Vel}}_i$ is initialised to a set of randomly generated integer values between $-|\mathbb{V}_\textit{res}|$ and $|\mathbb{V}_\textit{res}|$ (Alg.\ref{Algo1} Line~\ref{lineP5}). 

Next, the cost $\mathcal{C}_i$ of each $\vec{P}_i$ is computed by using Eq.\ref{eq:1} (Alg.\ref{Algo1} Line~\ref{lineP8}). The cost $\mathcal{C}_i$ represents the \emph{fitness function} for \textit{APSO}. Based on the obtained cost values, we can select $\eta$ set of solutions $\mathbb{P}_\textit{final}$ as shown in Alg.\ref{Algo1} Line~\ref{lineP11}. An additional parameter $\zeta$ is added which represents the objective of the algorithm (i.e., find a list of deployment solutions that $maximises$ or $minimises$ the fitness function and $\eta$). We choose the $\vec{P}_i$ with the optimal cost value as the global best solution $\vec{P}_\textit{best}^\textit{global}$ (Alg.\ref{Algo1} Line~\ref{lineP13}). 

\input{figuresTex/fig-pso1}

To find better deployment solutions (update $\vec{P}_i$ to $\vec{P}_{i}^\textit{new}$) \textit{APSO} uses \emph{four} vector variables, $\vec{P}_i$, $\vec{\textit{Vel}}_i$, $\vec{P}_i^\textit{local}$ and $\vec{P}_\textit{best}^\textit{global}$. First, it computes $\vec{\textit{Vel}}_{i}^\textit{new}$, which is the key variable to update $\vec{P}_i$, as \emph{three} variables influence it, as follows. $\omega$   defines how much $\vec{\textit{Vel}}_i$ can contribute to the updating process. $C1$ and $C2$ are the factors which affect  similarity between $\vec{P}_i^\textit{new}-\vec{P}_i^\textit{local}$ and $\vec{P}_i^\textit{new} - \vec{P}_\textit{best}^\textit{global}$ respectively. Two randomly generated variables $F1$ and $F2$ are used to reduce the bias introduced by $\vec{P}_i^\textit{local}$ and $\vec{P}_\textit{best}^\textit{global}$. Finally, the search space is restricted by using a modulo operation with $|\mathbb{V}_\textit{res}|$. 
Eq.\ref{eqVel} summarises the changes:
\begin{equation}
\label{eqVel}
\begin{array}{lcl}
\vec{\textit{Vel}}_i^\textit{new} 
&=& (\omega \cdot \vec{\textit{Vel}}_i  \\ 
&& ~+C1 \cdot F1 \cdot (\vec{P}_{i}^\textit{local} - \vec{P}_i) \\
&&  ~+C2 \cdot F2 \cdot (\vec{P}_\textit{best}^\textit{global} - \vec{P}_i)) \mod %\% 
|\mathbb{V}_\textit{res}| 
\end{array}
\end{equation}

Despite the novelty of our \textit{APSO} approach, the fundamental tasks performed by variables $C1$ and $C2$ in guiding particle movement and convergence remain unchanged. Therefore, to maintain alignment with established methodologies and ensure comparability with prior research, we opted to retain the variable values to \emph{two} as those used in past works \cite{bratton2007defining}. The values of $F1$ and $F2$ are generated randomly between $0$ and $1$ following a uniform distribution. The new deployment solution $\vec{P}_i^\textit{new}$ is computed using the existing solution $\vec{P}_i$ and the new $\vec{\textit{Vel}}_i^\textit{new}$, as shown in Eq.\ref{eqPos}:
\begin{equation}
\label{eqPos}
	\vec{P}_i^\textit{new} = (\vec{P}_i + \vec{\textit{Vel}}_i^\textit{new})\mod |\mathbb{V}_\textit{res}|   
\end{equation}

The new deployment solutions are checked and the cost for the valid solutions is calculated. 
If the new cost $\mathcal{C}_i^\textit{new}$ is better than the fitness value of $\vec{P}_{i}^\textit{local}$ and $\vec{P}_\textit{best}^\textit{global}$, it should be updated (Alg.\ref{Algo1} Line~\ref{lineP25}-\ref{lineP27}). 
Finally, we update the solutions $\mathbb{P}_\textit{final}$ by replacing the existing solutions with those in $\vec{P}^\textit{new}$ which have better cost values (Alg.\ref{Algo1} Line~\ref{lineP28}). The described steps (Alg.\ref{Algo1} Line~\ref{lineP14}-\ref{lineP27}) are repeated until the termination condition is met. 
 
\myparagraph{Termination} In this paper, \textit{terminate} is set to \textit{true}
after $100$ iterations or if there is no updating of the $\vec{P}_\textit{best}^\textit{global}$ in $30$ iterations. After the termination, $\mathbb{P}_\textit{final}$ is returned as output.
 
\input{algorithm/alg_apso.tex}

==> TC/relatedwork.tex <==
\section{Related work}
\label{sec:related}
We now provide a brief background of the benchmark applications and the benchmark orchestrators (\S~\ref{sec:background}). Following this, we discuss some related work (\S~\ref{sec:related}). Then, we illustrate the design goals to meet the new requirements of containerized web-applications which are not considered in any existing benchmark orchestrators (\S~\ref{sec:design-goal}). 

\subsection{Background}\label{sec:background}

To capture the behavior of web-applications, numerous benchmarks are proposed by academia \cite{scheuner2015cloud,chhetri2016smart,Cecchet:2011:BOT:2002168.2002172} and industry\footnote{https://cs.nyu.edu/~totok/professional/software/tpcw/tpcw.html}$^,${\footnote{https://www.wikibooks.org/} $^,$\footnote{https://cwiki.apache.org/confluence/display/OLIO/Index}}. These benchmarks try to emulate the server-side features of the application along with workload generation and injection. The server-side features are defined in terms of domain, different tiers and interactivity support \cite{Fielding:2017:RRA:3106237.3121282}. Multi-tier architecture support is provided in the form of MVC (Model View Controller) architecture which can be implemented using either traditional (e.g. JavaEE and ASP.NET) or modern (e.g. Python Django and Ruby on Rails) frameworks. Irrespective of the underlying framework, interactivity is supported by technologies such as jQuery, Angular and Underscore.js that ease the user interaction allowing personalization on different devices. 
Workload generation and injection that captures the user interaction behavior is an important component of a benchmark \cite{curiel2018workload}. 
Though a real trace-based benchmark \cite{Ratanaworabhan} can closely capture and mimic the  workload features, it is hard to generalize such benchmarks across multiple types of web applications. This is mainly due to the fact that a real trace can only represent a specific type of web application workload. Hence, there is need to find balance between generalizability and specificity during the benchmarking process.
%Using real data as a benchmark workload captures the best behavior however, it is specific only for particular application and is not easy to adapt or change according to the benchmark. 
This tension leads to the use of synthetic load generators that incorporates different user behaviors, e.g. think time and ramp up time to create sophisticated workloads \cite{4015510}. To maintain a continuous stream of load, the trace is repeated using some replay tool e.g. httperf\footnote{https://github.com/httperf/httperf} that sends the simple or customized trace (combination of different traces) to the application. 

%Benchmarks such as Wikibooks\footnote{https://www.wikibooks.org/} (for wikipedia), Cloudstone's Olio\footnote{https://cwiki.apache.org/confluence/display/OLIO/Index} (for social media), TPC-W\footnote{https://cs.nyu.edu/~totok/professional/software/tpcw/tpcw.html} (for transactional web e-Commerce) are specific for particular domain whereas Benchlab \cite{cecchet2011benchlab} can support multiple domains altogether.

The web-application benchmark needs to be deployed on various host configurations in the multi-cloud environment. Orchestrating the systematic deployment consists of following steps \cite{weerasiri2017taxonomy}: (i) defining the benchmark with their attributes and relationships, (ii) defining the host machine configuration (e.g., CPU cores, memory size, datacenter location, cost), (iii) instantiating the cloud host complying the application requirements, (iv) monitoring the resources to ensure the QoS and SLA parameters, and (v) controlling the overall processes. 

\subsection{Related work}\label{sec:related}
Performing all these steps manually is tedious, error-prone and requires a lot of time and diverse knowledge of architecture and accessing mechanism of all these environments. 
There are different frameworks available that automate/semi-automate the orchestration steps. 
%Some of the frameworks are cloud specific e.g. AWS CloudFormation\footnote{https://aws.amazon.com/cloudformation/} and Azure Resource Manager\footnote{https://azure.microsoft.com/en-gb/features/resource-manager/} while others are cloud agnostic e.g. Juju\footnote{https://jujucharms.com/}, Ansible\footnote{https://www.ansible.com/}. Frameworks such as Kubernetes (K8)\footnote{https://kubernetes.io/} and Docker Swarm\footnote{https://docs.docker.com/engine/swarm/} also handles the cluster management for containerized environment. 
%There are also some frameworks specific for benchmarking e.g. CloudBench \cite{silva2013cloudbench}, Smart CloudBench \cite{chhetri2016smart}. However, none of the above discussed frameworks consider the optimized selection of benchmark and time execution time of the benchmark within the defined budget. The main limitations of the above discussed work are summarized below.  
%Evaluating the system performance before the actual deployment has been studied extensively. TPC-W\footnote{https://cs.nyu.edu/~totok/professional/software/tpcw/tpcw.html}, WPBench \cite{zhang2009wpbench}, CloudStone \cite{sobel2008cloudstone}, Wikibooks\footnote{https://www.wikibooks.org/}, etc. are some common benchmarks for assessing the performance of web-application. Existing studies \cite{liew2012cloudguide,scheuner2018estimating,cecchet2011benchlab} uses these benchmarks to evaluate the performance of web-application in traditional VM environment. However, the containerized environment is different from the VM environment. 
%With the growing demand of containers, studies also benchmark the performance of containers. 
%Most of the existing studies 
\cite{felter2015updated,Sharma:2016,kozhirbayev2017performance} evaluated the performance of containers for scientific applications where a few of them \cite{xavier2014performance,zhang2018comparative} evaluate for big data applications. 
%However, in most of the works, the benchmarks configuration, host (VM/container) configuration and set up, benchmark execution and result collection is performed manually. 
However most of these works are intended for single cloud environment, without considering the complexity of interacting with various APIs/SDKs provided by different cloud providers. 
%It is not handy to perform all these operations by our own in multi-cloud environment as each cloud provider have specific APIs/SDKs for interaction. 

There are few existing frameworks that handle the orchestration of benchmarks in multi-cloud environment. CloudBench \cite{silva2013cloudbench} and Smart CloudBench \cite{chhetri2016smart} automates the benchmark execution in multi-cloud environment. However, it is not easy to define the benchmarks using these frameworks. Also they are not specific for containerized environment. Additionally, Varghese et al. proposed a framework called DocLite \cite{varghese2016doclite} to evaluate the performance of VMs using containerized microbenchmarks. Microbenchmarks are executed on different VMs and the ranking is evaluated by using the set of weights provided by the user for different system parameters. This framework is specific for scientific application and may not be applicable for web application. Our proposed SmartDBO orchestrates the benchmark for web-application while allowing users to define and deploy the benchmark in a very interactive and user-friendly way.

Additionally, there are some commercial tools,  e.g. CloudHarmony\footnote{https://cloudharmony.com/}, cloudorado\footnote{https://www.cloudorado.com/cloud\_server\_comparison.jsp}, Cloud Spectator \footnote{https://cloudspectator.com/}. available that perform the benchmark for users but they are not specific for particular applications. Also, they do not provide all the required metrics specific to that particular application for making proper decisions before final resource selection and provisioning. The limitations of the existing work are briefly summarized as follows.

%Performing benchmark is very expensive but none of the available work considers the cost of benchmark. Also, benchmarking host for long time gives more accurate evaluation but imposes high cost and is not always suggested. In this work, we are not only allowing the automatic orchestration of the benchmark but also furnish user to find a set of benchmark that can cover as much diversity as possible within the defined budget. Our benchmark orchestration is based on Infrastructure as a code that allows user to reuse the available code to ease their deployment. 


%\zy{review the important works related to web application benchmark and benchmark orchestrator}

\myparagraph{Limitations} The cloud providers provide the shared and virtualized computing resources to their customers, which makes the cloud environments dynamic and the SLA very hard to guarantee \cite{serrano2016sla}. Moreover, the web application is very sensitive to the dynamically changing environment that directly affect user's satisfaction. Capturing or monitoring the changing behavior of the cloud environments requires the users to run their benchmark applications over a considerable time, which is very costly.    
The existing benchmark applications/tools are not able to solve the trade-off between the limited budgets and the long-time benchmarking experiments.  

Additionally, the variety of cloud providers offer a massive configuration choices of host. For instance, Amazon EC2 provides $43$ types of host for their customers\footnote{https://aws.amazon.com/ec2/instance-types/} excluding self customized hosts. It is not possible to run the benchmark applications over all available resources. The state-of-the-art systems do not consider this case that provides an optimized recommendation to help users in selecting the hosts from the massive number of available hosts spanned across multiple cloud providers.

\subsection{Design goals}\label{sec:design-goal}

To overcome the limitations discussed in the previous subsection, our proposed \projecttitle framework follows the three main design goals:

\begin{itemize}
	\item We want to automatically orchestrate \emph{any} containerized benchmark application across multi-cloud environments based on the users' specification. This will remove the huge burden from user side, i.e. the users do not need to  manually deploy the benchmark applications and define the benchmark  plans  over various cloud datacenters.  
	\item We want to capture the dynamicity and the uncertainty of the cloud environment while ensuring the cost does not exceed the users' budget. This dynamicity and uncertainty may affect the performance of web-application, therefore reducing users'  satisfaction \cite{hoxmeier2000system}. 
%	For example,  This is important for web applications because the response time of a website is significantly affecting user satisfaction \cite{hoxmeier2000system}.  
	
	\item We should be able to find an optimal set of hosts for benchmarking in a fixed budget that covers the diversity, in terms of host configurations, both within a cloud provider and across the cloud providers. This feature improves the chance for a user to find the best mix of hosts for deploying their web-applications. In other words, with our design the users has more chance to find the cheaper hosts which meet the performance requirements of their web applications. 
\end{itemize}

%\input{figuresTex/fig-shortterm}

%\input{figuresTex/fig-longterm}





